Late-time HST and JWST Observations of GRB 221009A: Evidence for a Break in the Light Curve at 50 Days

GRB 221009A is one of the brightest transients ever observed with the highest peak gamma-ray flux for a gamma-ray burst (GRB). A type Ic-BL supernova (SN), SN 2022xiw, was definitively detected in late-time JWST spectroscopy (t = 195 days, observer-frame). However, photometric studies have found SN 2022xiw to be less luminous (10-70%) than the canonical GRB-SN, SN 1998bw. We present late-time Hubble Space Telescope (HST)/WFC3 and JWST/NIRCam imaging of the afterglow and host galaxy of GRB 221009A at t ~ 185, 277, and 345 days post-trigger. Our joint archival ground, HST, and JWST light curve fits show strong support for a break in the light curve decay slope at t = 50 +/- 10 days (observer-frame) and a supernova at $< 1.5 \times$ the optical/NIR flux of SN 1998bw. This break is consistent with an interpretation as a jet break when requiring slow-cooling electrons in a wind medium with the electron energy spectral index, p > 2, and $\nu_m < \nu_c$. Our light curve and joint HST/JWST spectral energy distribution (SED) also show evidence for the late-time emergence of a bluer component in addition to the fading afterglow and supernova. We find consistency with the interpretations that this source is either a young, massive, low-metallicity star cluster or a scattered light echo of the afterglow with a SED shape of $f_{\nu} \propto \nu^{2.0\pm1.0}$.

==> authors.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Moved to main.tex
% Please make changes there
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\author[0000-0001-8023-4912]{Huei Sears}
\affiliation{Department of Physics and Astronomy, Rutgers, the State University of New Jersey, 136 Frelinghuysen Road, Piscataway, NJ 08854-8019, USA}

\author[0000-0002-7706-5668]{Ryan Chornock}
\affiliation{Department of Astronomy, University of California, Berkeley, CA 94720-3411, USA}

\author[0000-0003-0526-2248]{Peter K. Blanchard}
\affiliation{Center for Astrophysics \textbar\ Harvard \&\ Smithsonian, 60 Garden Street, Cambridge, MA 02138-1516, USA}

\author[0000-0003-4768-7586]{Raffaella Margutti}
\affiliation{Department of Astronomy, University of California, Berkeley, CA 94720-3411, USA}
\affiliation{Department of Physics, University of California, 366 Physics North MC 7300, Berkeley, CA 94720, USA}

\author[0000-0002-5814-4061]{V.~Ashley Villar}
\affiliation{Center for Astrophysics \textbar\ Harvard \&\ Smithsonian, 60 Garden Street, Cambridge, MA 02138-1516, USA}
\affiliation{The NSF AI Institute for Artificial Intelligence and Fundamental Interactions}

\author[0000-0002-2361-7201]{Justin Pierel}
\altaffiliation{NHFP Einstein Fellow}
\affiliation{Space Telescope Science Institute, Baltimore, MD 21218, USA}

\author[0000-0001-5661-7155]{Patrick J. Vallely}
\affiliation{Core Pricing Systems, CarMax, Inc., Richmond, VA 23238, USA}

%%%%%%%%%%%%%%%%%%%
%HST + JWST CoIs
%%%%%%%%%%%%%%%%%%%

\author[0000-0002-8297-2473]{Kate D.~Alexander}
\affiliation{Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA}

\author[0000-0002-9392-9681]{Edo Berger}
\affiliation{Center for Astrophysics \textbar\ Harvard \&\ Smithsonian, 60 Garden Street, Cambridge, MA 02138-1516, USA}
\affiliation{The NSF AI Institute for Artificial Intelligence and Fundamental Interactions}

\author[0000-0003-0307-9984]{Tarraneh~Eftekhari}
\altaffiliation{NHFP Einstein Fellow}
\affiliation{Center for Interdisciplinary Exploration and Research in Astronomy (CIERA), Northwestern University, 1800 Sherman Avenue, Evanston, IL 60201, USA}

\author[0000-0002-3934-2644]{Wynn ~V.~Jacobson-Gal\'{a}n}
\altaffiliation{NASA Hubble Fellow}
\affil{Department of Astronomy and Astrophysics, California Institute of Technology, Pasadena, CA 91125, USA}

\author[0000-0003-1792-2338]{Tanmoy Laskar}
\affiliation{Department of Physics \& Astronomy, University of Utah, Salt Lake City, UT 84112, USA}
\affiliation{Department of Astrophysics/IMAPP, Radboud University, P.O. Box 9010, 6500 GL, Nijmegen, The Netherlands}

\author[0000-0002-2249-0595]{Natalie LeBaron}
\affiliation{Department of Astronomy, University of California, Berkeley, CA 94720-3411, USA}

\author[0000-0002-4670-7509]{Brian D.~Metzger}
\affil{Department of Physics and Columbia Astrophysics Laboratory, Columbia University, New York, NY 10027, USA}
\affil{Center for Computational Astrophysics, Flatiron Institute, 162 5th Ave, New York, NY 10010, USA}

\author[0000-0002-0763-3885]{Dan Milisavljevic}
\affiliation{Department of Physics and Astronomy, Purdue University, 525 Northwestern Ave, West Lafayette, IN 47907, USA}

%%%%%%%%%%%
% Opted Out
%%%%%%%%%%%
% \author[]{Jenni Barnes}
% \affiliation{}

% \author[]{Yvette Cendes}
% \affiliation{}

% \author[]{Joel Leja}
% \affiliation{}

% \author[]{S. Karthik Yadavalli}
% \affiliation{}

%%%%%%%%%%%
% Did not reply
%%%%%%%%%%%

% \author[]{Dan Kasen}
% \affiliation{}

% \author[]{Dan Siegel}
% \affiliation{}
